Performance-Robustness Tradeoffs in Adversarially Robust Control and Estimation

While $\mathcal{H}_\infty$ methods can introduce robustness against worst-case perturbations, their nominal performance under conventional stochastic disturbances is often drastically reduced. Though this fundamental tradeoff between nominal performance and robustness is known to exist, it is not well-characterized in quantitative terms. Toward addressing this issue, we borrow the increasingly ubiquitous notion of adversarial training from machine learning to construct a class of controllers which are optimized for disturbances consisting of mixed stochastic and worst-case components. We find that this problem admits a linear time invariant optimal controller that has a form closely related to suboptimal $\mathcal{H}_\infty$ solutions. We then provide a quantitative performance-robustness tradeoff analysis in two analytically tractable cases: state feedback control, and state estimation. In these special cases, we demonstrate that the severity of the tradeoff depends in an interpretable manner upon system-theoretic properties such as the spectrum of the controllability gramian, the spectrum of the observability gramian, and the stability of the system. This provides practitioners with general guidance for determining how much robustness to incorporate based on a priori system knowledge. We empirically validate our results by comparing the performance of our controller against standard baselines, and plotting tradeoff curves.

==> tac.tex <==
% \documentclass[journal,twoside,web]{ieeecolor}
% \usepackage{generic}
% % \usepackage{cite}
% \usepackage{amsmath,amssymb,amsfonts}

% \usepackage{graphicx}
% \usepackage{algorithm}
% \usepackage{algpseudocode}
% % \usepackage{hyperref}
% % \hypersetup{hidelinks=true}
% \usepackage{textcomp}
% \def\BibTeX{{\rm B\kern-.05em{\sc i\kern-.025em b}\kern-.08em
%     T\kern-.1667em\lower.7ex\hbox{E}\kern-.125emX}}
% \markboth{\hskip25pc IEEE TRANSACTIONS AND JOURNALS TEMPLATE}
% {Lee \MakeLowercase{\textit{et al.}}: Performance-Robustness Tradeoffs in Adversarially Robust Control and Estimation}


% \usepackage{caption}
% \usepackage{subcaption}

% \usepackage{calc}
% \usepackage{bm, tabularx}
% \usepackage{latexsym, mathtools}
% \usepackage{cleveref}
% \usepackage{thmtools} 
% \usepackage{thm-restate}

% \usepackage{Shorthands}

% \newcommand{\citep}[1]{\cite{#1}}

% \newcommand{\hh}[1]{\noindent{\textcolor{blue}{\textbf{HH:} \textsf{#1} }}}
% % \usepackage{cleveref}
% % \usepackage{thmtools} 
% % \usepackage{thm-restate}

% \title{Performance-Robustness Tradeoffs in Adversarially Robust Control and Estimation}

% \author{Bruce D.\ Lee, \IEEEmembership{Student Member, IEEE}, Thomas T.C.K.\ Zhang, \IEEEmembership{Student Member, IEEE}, Hamed Hassani, \IEEEmembership{Member, IEEE}, and Nikolai Matni, \IEEEmembership{Member, IEEE} \thanks{Submitted on May 26, 2023. Bruce D.\ Lee is supported by the DoD through the National Defense Science \& Engineering Graduate Fellowship Program. The research of Hamed Hassani is supported by NSF Grants 1837253, 1943064, 1934876, AFOSR Grant FA9550-20-1-0111, and DCIST-CRA. Nikolai Matni is funded by NSF awards CPS-2038873, CAREER award ECCS-2045834, and ECCS-2231349. } \thanks{All authors are with the Department of Electrical and Systems Engineering at the University of Pennsylvania (e-mails: \{brucele, ttz2, hassani, nmatni\}@seas.upenn.edu). }}

% \date{Department of Electrical and Systems Engineering, University of Pennsylvania}

% \newcounter{tac}
% \setcounter{tac}{1}

% \begin{document}

% \maketitle
% \input{abstract}
% \input{introduction}
% \input{adversariallyrobustcontrol}
% \input{Nominaltradeoffs_statefeedback}
% \input{Nominaltradeoffs_kalmanfiltering}
% \input{empirical}
% \input{conclusion}


% \section*{REFERENCES}
% \bibliographystyle{IEEEtran}
% \bibliography{refs}
% \vspace{-0.5in}
% \begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{figures/bruce.jpg}}]{Bruce D. Lee,} (Student Member, IEEE), is a Ph.D. student in the Department of Electrical and Systems Engineering at the University of Pennsylvania. He also holds a B.E.E. from the University of Minnesota, Twin Cities. 
% \end{IEEEbiography}
% \
% \begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{figures/thomas.jpeg}}]{Thomas T.C.K. Zhang,} (Student Member, IEEE), is a Ph.D. student in the Department of Electrical and Systems Engineering at the University of Pennsylvania. He also holds B.S. degrees in mathematics and statistics \& data science from Yale University. 
% \end{IEEEbiography}
% \begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{figures/hassani-hamed.jpg}}]{Hamed Hassani,} (Member, IEEE), is an Assistant Professor in the Department of Electrical and Systems Engineering. He holds secondary appointments in the Department of Computer and Information Systems as well as the Department of Statistics and Data Science at the Wharton Business School. He is also a faculty affiliate of the Warren Center for Network and Data Sciences. 
% Before joining Penn, he was a research fellow at the Simons Institute, UC Berkeley. Prior to that, he was a post-doctoral scholar and lecturer in the Institute for Machine Learning at ETH Zürich. He received his Ph.D. degree in Computer and Communication Sciences from EPFL. 
% \end{IEEEbiography}
% \begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{figures/nik.jpg}}]{Nikolai Matni,} (Member, IEEE), is an Assistant Professor in the Department of Electrical and Systems Engineering at the University of Pennsylvania, with a secondary appointment in Computer and Information Sciences. He is also a member the Applied Mathematics and Computaitonal Science graduate group. Prior to joining The University of Pennsylvania, Nikolai was a postdoctoral scholar in EECS at UC Berkeley. He has also held a position as a postdoctoral scholar in the Computing and Mathematical Sciences at Caltech. He received his Ph.D. in Control and Dynamical Systems from Caltech in June 2016. He also holds B.A.Sc. and M.A.Sc. in Electrical Engineering from the University of British Columbia, Vancouver, Canada. His research interests broadly encompass the use of learning, optimization, and control in the design and analysis of safety-critical and data-driven cyber-physical systems.
% \end{IEEEbiography}


% \end{document}

 
